A new definition of analytic adjoint ideal sheaves via the residue functions of log-canonical measures I

A new definition of analytic adjoint ideal sheaves for quasi-plurisubharmonic (quasi-psh) functions with only neat analytic singularities is studied and shown to admit some residue short exact sequences which are obtained by restricting sections of the newly defined adjoint ideal sheaves to some unions of $\sigma$-log-canonical ($\sigma$-lc) centres. The newly defined adjoint ideal sheaves induce naturally some residue $L^2$ norms on the unions of $\sigma$-lc centres which are invariant under log-resolutions. They can also describe unions of $\sigma$-lc centres without the need of log-resolutions even if the quasi-psh functions in question are not in a simple-normal-crossing configuration. This is hinting their potential use in discussing the $\sigma$-lc centres even when the quasi-psh functions in question have more general singularities. Furthermore, their relations between the algebraic adjoint ideal sheaves of Ein--Lazarsfeld as well as those of Hacon--McKernan are described in order to illustrate their role as a (potentially finer) measurement of singularities in the minimal model program. In the course of the study, a local $L^2$ extension theorem is proven, which shows that holomorphic sections on any unions of $\sigma$-lc centres can be extended holomorphically to some neighbourhood of the unions of $\sigma$-lc centres with some $L^2$ estimates. The proof does not rely on the techniques in the Ohsawa--Takegoshi-type $L^2$ extension theorems.

==> mariostdcommands.tex <==
%%%%%
%%%%% File name  : mariostdcommands.tex
%%%%% Author     : Mario Chan
%%%%% Last update: 2nd September, 2022
%%%%% Description: Math LaTeX command definitions (without packages)
%%%%%              used by Mario Chan.
%%%%%
%%
%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin of definitions of commands 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\newcommand{\fieldC}{\mathbb{C}}
\newcommand{\fieldR}{\mathbb{R}}
\newcommand{\fieldQ}{\mathbb{Q}}
\newcommand{\Znum}{\mathbb{Z}}
\newcommand{\Nnum}{\mathbb{N}}
\newcommand{\Nnump}{\mathbb{N}_{>0}}
%\newcommand{\Onum}{\mathfrak{o}}
%\newcommand{\Cl}{\mathscr{C}\!\mathpzc{l}}
\newcommand{\Zmod}[1]{\Znum/#1\Znum}

\newcommand{\cplxi}{\sqrt{-1}}
% \newlength{\ibarbarheight}
% \setlength{\ibarbarheight}{-0.9ex}
% \newcommand{\ibar}{{\raisebox{\ibarbarheight}{$\mathchar'26$}\mkern-6.7mu i}}
\newcommand{\ibar}{
  \smash[b]{
    \begin{tikzpicture}[trim left, baseline=0pt]
      \node (i) [anchor=base, text width=0pt, text height=0pt] {$i$};
      \node (bar) [below left=0.75ex and 0.12ex, inner sep=0pt,
      outer sep=0pt, text width=0ex, text height=0ex] {$\mathchar'26$};
    \end{tikzpicture}
  }
}
\newcommand{\ibardefn}{\frac{\cplxi}{2\pi}}
\newsavebox{\ibarExplainBox}
\begin{lrbox}{\ibarExplainBox}
  \footnotesize
  \verb:{\raisebox{-0.9ex}{$\mathchar'26$}\mkern-6.7mu i}: 
\end{lrbox}
\newcommand{\ibarfootnote}{\footnote{The notation is chosen by
    mimicking the reduced Planck constant $\hbar = \frac{h}{2\pi}$. It
    can be typeset with the code \usebox\ibarExplainBox.}}
\newcommand{\proj}{\mathbb{P}}
\newcommand{\sphere}{\mathbb{S}}
\newcommand{\uhp}{\mathfrak{H}}
\newcommand{\eps}{\varepsilon}
\newcommand{\vphi}{\varphi}

\newcommand{\sheaf}[1]{\mathscr{#1}}
\newcommand{\ideal}[1]{\mathfrak{#1}}
\newcommand{\bundle}[1]{\mathbb{#1}}

\newcommand{\mero}{\sheaf{M}}
\newcommand{\holo}{\sheaf{O}}
\newcommand{\holoform}{\boldsymbol\Omega}
\newcommand{\kanshf}[1][X]{\sheaf K_{#1}}
\newcommand{\smooth}[1][\infty]{\mathscr C^{#1}}
\NewDocumentCommand{\smform} { s D//{p,q} O{X} }{
  \sheaf A^{#2}_{#3\IfBooleanT{#1}{\,c}}  
}
\newcommand{\Lloc}[1][1]{L^{#1}_{\text{loc}}}
\newcommand{\maxidl}{\ideal m}
\newcommand{\multidl}{\sheaf I}

\NewDocumentCommand{\Tgt}{ %% Tangent bundle
  s       %% #1 turn to cotangent bundle when starred
  d//     %% #2 types of (co)tangent vectors wrt almost cplx structure
}{\mathbf T^{\IfBooleanT{#1}{*\IfNoValueF{#2}{\,}}\IfNoValueF{#2}{#2}}}

\def\cTgt{\Tgt*} %% Cotangent bundle, for backward compatibility

% \newcommand{\Tgt}[1][]{\mathbf T^{#1}}
% \newcommand{\cTgt}[1][]{\Tgt[*\,#1]}

\NewDocumentCommand{\cohgp}{
  O{H}   %% #1 symbol for cohomology (e.g.~H or \check H)
  t_     %% #2 with "_", it becomes homology
  m      %% #3 (co)homology degree
  D<>{}  %% #4 sub/super-scripts to be put to the (co)homology group
  o      %% #5 supporting space
  D//{,} %% #6 separator between space and coefficients 
  m      %% #7 coefficients
}{
  #1\IfBooleanTF{#2} {_{#3}^{#4}} {^{#3}_{#4}} \paren{\IfNoValueF{#5}{#5#6} #7}
}

\NewDocumentCommand{\cohdim}{
  t_     %% with "_", it becomes homology
  m      %% (co)homology degree
  D<>{}  %% sub/super-scripts to be put to the (co)homology group
  o      %% supporting space
  D//{,} %% separator between space and coefficients 
  m      %% coefficients
}{
  h\IfBooleanTF{#1} {_{#2}^{#3}} {^{#2}_{#3}} \paren{\IfNoValueF{#4}{#4#5} #6}
}

\newcommand{\codim}{\operatorname{codim}}
\newcommand{\Sing}{\operatorname{Sing}}
\newcommand{\mult}{\operatorname{mult}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\pr}{\operatorname{pr}}
\newcommand{\Tr}{\operatorname{Tr}}
\newcommand{\rk}{\operatorname{rk}}
\newcommand{\vol}{\operatorname{vol}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\Dom}{\operatorname{Dom}}
\newcommand{\Alb}{\operatorname{Alb}}
\newcommand{\alb}{\operatorname{alb}}
\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Exc}{\operatorname{Exc}}
\newcommand{\Hess}{\operatorname{Hess}}
\newcommand{\esssup}{\operatorname*{ess\,sup}}
\newcommand{\BigO}{\operatorname{\mathbf{O}}}

% \newcommand{\bexp}{\boldsymbol{\operatorname{e}}}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}

\newcommand{\symmgp}{\mathfrak{S}}
\newcommand{\GL}[2][2]{\mathrm{GL}_{#1}(#2)}
\newcommand{\SL}[2][2]{\mathrm{SL}_{#1}(#2)}
\newcommand{\SO}[2][2]{\mathrm{SO}_{#1}(#2)}
% \newcommand{\SL}[1]{\mathrm{SL}_2(#1)}
% \newcommand{\SO}[1]{\mathrm{SO}_2(#1)}
\newcommand{\SU}[1]{\mathrm{SU}(#1)}
\newcommand{\Aut}[1]{\mathrm{Aut}(#1)}
\newcommand{\Div}[1]{\mathrm{Div}(#1)}
\newcommand{\divsr}[1]{\mathrm{div}\paren{#1}}

\newcommand{\sgn}[1]{\operatorname{sgn}(#1)}

%%%%% Could be replaced by calling the package "mleftright" 
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}
%%%%%

\newcommand{\lparpht}[2][(]{\mathopen{\left#1\vphantom{#2}\right.\kern-\nulldelimiterspace}}
\newcommand{\rparpht}[2][)]{\mathclose{\left.\kern-\nulldelimiterspace\vphantom{#2}\right#1}}
% \newcommand{\lparpht}[1]{\mathopen{\left(\vphantom{#1}\right.\kern-\nulldelimiterspace}}
% \newcommand{\rparpht}[1]{\mathclose{\left.\kern-\nulldelimiterspace\vphantom{#1}\right)}}
% \newcommand{\paren}[1]{\!\left(#1\right)}
\newcommand{\paren}[1]{\lparpht{#1}#1\rparpht{#1}}
\newcommand{\bigparen}[1]{\bigl(#1\bigr)}
\newcommand{\res}[1]{\left.#1\right|}
\newcommand{\parres}[1]{\res{\paren{#1}}}
\newcommand{\seq}[1]{\lparpht[\{]{#1}#1\rparpht[\}]{#1}}
% \newcommand{\seq}[1]{\left\{#1\right\}}
\newcommand{\set}[1]{\lparpht[\{]{#1}#1\rparpht[\}]{#1}}
% \newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\setd}[2]{\left\{#1\:\left|\;\vphantom{#1} #2\right.\right\}}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigabs}[1]{\bigl\lvert#1\bigr\rvert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bignorm}[1]{\bigl\lVert#1\bigr\rVert}
\newcommand{\Bignorm}[1]{\Bigl\lVert#1\Bigr\rVert}
\newcommand{\inner}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\ptinner}[2]{\left(#1,#2\right)}
\newcommand{\biginner}[2]{\bigl\langle#1,#2\bigr\rangle}
\newcommand{\commut}[2]{\left[#1,#2\right]}
\newcommand{\algnorm}[1]{\mathbf N(#1)}
\newcommand{\smod}[1]{\,(\operatorname{mod}\,#1)}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\Ceil}[1]{\bigl\lceil#1\bigr\rceil}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\fracpart}[1]{\left\{#1\right\}}

\newcommand{\tp}[1]{\,{\vphantom{#1}}^*\! #1}
\newcommand{\rtp}[1]{\,{\vphantom{#1}}^t\! #1}

\newcommand{\genby}[1]{\left\langle#1\right\rangle}
\newcommand{\genbyd}[2]{\left\langle#1\:\left|\;\vphantom{#1} #2\right.\right\rangle}

\newcommand{\tmatrix}[4]{\left[\begin{smallmatrix}#1 & #2 \\ #3 & #4\end{smallmatrix}\right]}
\newcommand{\Diag}[1]{\operatorname{diag}\bigl(#1\bigr)}

\newcommand{\cl}{\overline}

\newcommand{\vect}[1]{\underline{#1}}

\newcommand{\conj}{\overline}
\newcommand{\diff}{\partial}
%% \dbar is defined in amsrefs (mathscinet) with out 'lite' option, so
%% \renewcommand is used 
\makeatletter
\@ifundefined{dbar}{
  \newcommand{\dbar}{{\conj\diff}}  
}{
  \renewcommand{\dbar}{{\conj\diff}}
  % \PackageWarningNoLine{marionotations}{`\protect\dbar' is redefined}
  \@latex@warning@no@line{`\protect\dbar' is redefined in mariostdcommands.tex}
}
\makeatother

\NewDocumentCommand{\fdiff}{O{#3} m O{}}{\frac{\diff #1}{\diff #2}}
\newcommand{\dfadj}{\vartheta}
\newcommand{\ddbar}{\diff\dbar}
\newcommand{\iddbar}{\cplxi\ddbar}
\newcommand{\ibddbar}{\ibar\ddbar}

\newcommand{\ddc}{dd^c\mspace{1mu}}

\newcommand{\bdry}{\partial}

\newcommand{\birat}{\mathrel{\dashrightarrow}}
\newcommand{\tendsto}{\mathrel{\rightarrow}}
\newcommand{\xtendsto}[1]{\mathrel{\xrightarrow{#1}}}
\newcommand{\wktendsto}{\mathrel{\rightharpoonup}}
\newcommand{\descendsto}{\mathrel{\searrow}}
\newcommand{\ascendsto}{\mathrel{\nearrow}}
\newcommand{\imply}{\mathrel{\Rightarrow~}}
\newcommand{\isom}{\mathrel{\cong}}
\newcommand{\ctrt}{\mathbin{\lrcorner}}


